Free-stream preserving finite difference schemes for ideal magnetohydrodynamics on curvilinear meshes

In this paper, a high order free-stream preserving finite difference weighted essentially non-oscillatory (WENO) scheme is developed for the ideal magnetohydrodynamic (MHD) equations on curvilinear meshes. Under the constrained transport framework, magnetic potential evolved by a Hamilton-Jacobi (H-J) equation is introduced to control the divergence error. In this work, we use the alternative formulation of WENO scheme [10] for the nonlinear hyperbolic conservation law, and design a novel method to solve the magnetic potential. Theoretical derivation and numerical results show that the scheme can preserve free-stream solutions of MHD equations, and reduce error more effectively than the standard finite difference WENO schemes for such problems.

==> title.tex <==
\begin{center}
{\bf
%>> A Kernel Based High Order \lq\lq Explicit'' Unconditionally Stable Scheme for Time Dependent Hamilton-Jacobi Equations
 A Kernel Based High Order \lq\lq Explicit'' Unconditionally Stable Constrained Transport Method for Ideal Magnetohydrodynamics 
}
\end{center}

\vspace{.2in}
\centerline{
Andrew Christlieb\footnote{
 Department of Computational Mathematics, Science and Engineering, Department of Mathematics  and  Department of Electrical Engineering, Michigan State University, East Lansing, MI, 48824. E-mail: christli@msu.edu
},
Firat Cakir \footnote{Department of Mathematics, Michigan State University, East Lansing, MI, 48824. E-mail: cakirfir@msu.edu},
and 
Yan Jiang\footnote{School of Mathematical Sciences, University of Science and Technology of China, Hefei, Anhui 230026, People's Republic of China. E-mail: jiangy@ustc.edu.cn }
}

\bigskip
\noindent
{\bf Abstract.}


The ideal Magnetohydrodynamics (MHD) equations are challenging because one needs to maintain the divergence free condition, $\nabla \cdot \Bv = 0$. Many numerical methods have been developed to enforce this condition. In this current work, we further our work on mesh aligned constraint transport by developing a new Kernel based approach for the vector potential in 2D and 3D. The approach for solving the vector potential is based on the method of lines transpose  and is A-stable, eliminating the need for diffusion limiters needed in our previous work in 3D. The work presented here is an improvement over the previous method in the context of problems with strong shocks due to the fact that we could eliminate the diffusion limiter that was needed in our previous version of constraint transport. The method is robust and has been tested on the 2D and 3D cloud shock, blast wave and field loop problems.

%*******Alternatif Cumleler****************
% 1. The ideal Magnetohydrodynamics (MHD) equations are one of the most important model of plasma physics. A significant challenge in the field of MHD simulations is to maintain the divergence free condition...Many numerical methods have been proposed for simulating MHD flows.
% 2. ensuring divB=0.
%
%**********************************************

%*******Alternatif Cumleler*********ref-20*******
% 1. Numerical methods for solving the ideal magnetohydrodynamics equations confront a significant challenge of satisfying the divergence free condition for magnetic field. 
% 2. One approach for maintaining that condition is through a so-called constraint transport method, which is based on first predicting a magnetic field through a standard finite volume solver, and then correcting this field through the appropriate use of a magnetic vector potential. 
%***************************************************
%*******Alternatif Cumleler*********ref-20*******
% 1. CT schemes can be viewed as predictorcorrector methods for updating the magnetic field, where a magnetic field value is first predicted by a method that does not exactly preserve the divergence-free condition on the magnetic field, followed by a correction step that aims to control these divergence errors.

\vfill

{\bf Key Words:} Magnetohydrodynamics; Constrained transport; Kernel based scheme; High order accuracy; Plasma physics. %Weighted essentially non-oscillatory methodology.

\newpage

